Not Just Skipping. Understanding the Effect of Sponsored Content on Users' Decision-Making in Online Health Search

Advertisements (ads) are an innate part of search engine business models. Advertisers are willing to pay search engines to promote their content to a prominent position in the search result page (SERP). This raises concerns about the search engine manipulation effect (SEME): the opinions of users can be influenced by the way search results are presented. In this work, we investigate the connection between SEME and sponsored content in the health domain. We conduct a series of user studies in which participants need to evaluate the effectiveness of different non-prescription natural remedies for various medical conditions. We present participants SERPs with different intentionally created biases towards certain viewpoints, with or without sponsored content, and ask them to evaluate the effectiveness of the treatment only based on the information presented to them. We investigate two types of sponsored content: 1. Direct marketing ads that directly market the product without expressing an opinion about its effectiveness, and 2. Indirect marketing ads that explicitly advocate the product's effectiveness on the condition in the query. Our results reveal a significant difference between the influence on users from these two ad types. Though direct marketing ads are mostly skipped by users, they can tilt users decision making towards more positive viewpoints. Indirect marketing ads affect both the users' examination behaviour and their perception of the treatment's effectiveness. We further discover that the contrast between the indirect marketing ads and the viewpoint presented in the organic search results plays an important role in users' decision-making. When the contrast is high, users exhibit a strong preference towards a negative viewpoint, and when the contrast is low or none, users exhibit preference towards a more positive viewpoint.

==> Ads paper arXiv/archive.tex <==


%\begin{table}
%\caption{T-Tests comparisons between the different answers for all ad-bias configurations}
%\vspace{-1mm}
% \begin{tabular}{|c|c|c|c|c|}
%\cline{2-5}
%\multicolumn{1}{c|}{}&\thead{df}&\thead{Yes-\\Maybe}&\thead{Yes-\\No}&\thead{Maybe-\\No}\\
%\hline
%\textbf{Y}&53&t=4.31,p < 0.01&t=4.72,p < 0.01&t=1.43,p > 0.05\\
%\hline
%\textbf{AY}&32&t=1.00,p > 0.05&t=4.00,p < 0.01&t=3.73,p < 0.01\\
%\hline
%\textbf{SY}&33&t=-1.00,p > 0.05&t=3.45,p < 0.01&t=3.71,p < 0.01\\
%\hline
%\hline
%\textbf{M}&49&t=-4.15,p < 0.01&t=-1.00,p > 0.05&t=3.93,p < 0.01\\
%\hline
%\textbf{AM}&42&t=-3.33,p < 0.01&t=-1.00,p > 0.05&t=3.10,p < 0.01\\
%\hline
%\textbf{SM}&63&t=-1.43,p > 0.05&t=4.01,p < 0.01&t=4.39,p < 0.01\\
%\hline
%\hline
%\textbf{N}&49&t=-4.58,p < 0.01&t=-4.37,p < 0.01&t=1.00,p > 0.05\\
%\hline
%\textbf{AN}&45&t=-2.60,p < 0.05&t=-3.54,p < 0.01&t=-2.07,p < 0.05\\
%\hline
%\textbf{SN}&51&t=-2.33,p < 0.05&t=-5.65,p < 0.01&t=-4.55,p < 0.01\\
%\hline
%\end{tabular}
%\label{tab:ttest}
%\vspace{-3mm}
%\end{table}



%When the maximal bias level of SERPs is towards the negative viewpoint we see that when no ads are present the `No' and and `Maybe' answers receive a similar percentage of the answers while the `Yes' answer receives a significantly lower percentage. Indicating that partipants had a difficult time interpreting the negative content. When referring to scientific evidence, as in query topics discussed in this study, negative content can often discuss existing positive findings while presenting an overall negative conclusion. This can confuse layman readers. For direct marketing ads we see a similar portion of negative answers but the division of the remaining responses is no longer similar with the `Maybe' response receiving significantly higher portion of the responses in comparison to the `Yes' answer. We see a similar phenomena in the indirect marketing ads setting. However, in this setting we see an significant increase in the portion of users selecting ``No'', both in comparison to the other two answers and to the portion of users selecting ``No'' in the no ads and direct marketing ads configuration. We hypothesis that the difference between the reaction to both ad types stems from the explicit nature of indirect marketing which had a different effect of partipants that were perhaps dangling between two possible answers. Since direct marketing ads don't explicitly express an opinion regarding treatments' effectiveness they did not elicit significant negative bias with those unsure partipants.Participants that were otherwise inclined to select ``Maybe'', perhaps dangling between ``Yes'' and ``Maybe'', were positively affected by the ad and chose ``Yes''. As opposed to indirect marketing ads that explicitly praised the treatment, in the title and snippet of their sponsored web page, causing those dangling  between ``Maybe'' and ``No'' to choose no.  

 

%existence of the indirect marketing content introduced negative sentiments to partipants, causing those unsure partipants, that might have chosen a ``Maybe'' response in the No ads configuration, to opt for the ``No'' response.  
%Though according to the CTR information for negative bias SERPs both the direct or indirect marketing ads were generally skipped.

%Unlike the the positive and inconclusive bias, where the no ads configuration the most popular response correlated to the viewpoint bias. 




%When the maximal bias level is towards the positive viewpoint and no ads are present the ``Yes'' answer is chosen by most participants at a percentage which is quite higher than that of partipants that chose either ``Maybe'' or ``No''. . A different behaviour is exhibited when ads are present. In both the direct and indirect marketing ad configurations, we see a  higher portion of partipants choosing the ``Maybe'' in comparison to the no ads configurations. This difference is  weakly significant in the direct marketing ads configuration t(85.0)=-1.6, p=0.056,  and strongly significant difference in the indirect marketing ads configuration t(86.0)=-1.78, p=0.039.  These results indicate that for positive bias SERPs, where the viewpoint presented by the ads correlates to viewpoint ranking bias expressed in the SERP, participants that consumed negative viewpoint content were effected not only by the ranking bias of the SERP in general but also by the ads and opted for a ``Maybe'' response more frequently.  And this occurred  whether or not they consumed the content in the ad. 



%When the maximal bias level of SERPs is towards the inconclusive viewpoint we see that when no ads are present the correlating `Maybe' response received the highest portion of answers.  When examining the ads configurations for this bias level, we see different behaviours between the direct and indirect marketing configuration. When direct marketing ads are present we see a similar behaviour to that of the no ads configuration. However for the indirect marketing ads we see that the ``Yes'' response receives a significantly higher portion of responses in comparison toe the no ads configuration, t(112.0)=-1.71, p=0.045.We hypothesize that since the viewpoint of the SERP was not definite, participants were not effected by direct marketing ads. This might be due to to the fact that its opinion regarding the treatments effectiveness is very implicit. They were however effected by the indirect marketing ads where we see a lower percentage of negative answers and a higher percentage of positive answers.
%We see a general shift towards more positive answers. We hypothesise that participants that were exposed to the ad in addition to negative content were more likely to chose the `'Maybe'' answer and participants that exposed to the ad in addition to inconclusive results were more prone to choose ``Yes''.

%When the maximal bias level of SERPs is towards the negative viewpoint we see that when no ads are present the `No' and and `Maybe' answers receive a similar percentage of the answers while the `Yes' answer receives a significantly lower percentage.  For direct marketing ads we do not see any sadistically significant difference between the different response percentages. However, for indirect marketing ads we see a weakly significantly higher percentage of negative responses in comparison to that of the no ads configuration. t(100)=-1.4,p=0.08 and a strongly significant for the `Maybe' response t(100)=1.8,p=0.04. This, despite of the fact that according to the CTR information for negative bias SERPs both the direct or indirect marketing ads were generally skipped. Meaning that the indirect marketing ad invoked a negative sentiment amongst partipants that caused partipants that were exposed to inconclusive content opted to select a negative answer more often, simply by noticing that the ad existed, event without inspecting it. This did not occur in the direct marketing setting. In fact we even see a slighr inclination towards a more positive restuls 


%Despite the fact that according to the CTR data, participants did enter the sponsored and the sponsored content expressed the same viewpoint as the organic result. The meet fact that sponsored content existed in the SERP. When an ad is present the rank of each organic results is pushed one position down. Before encounterin a negative or an oncoclusive result viewpoint the partipant is present with ate least one positove viewpoint results and the ad which is also considred as intoducing a positive viewpoint. Since there is no contradiction between the viewpoint bias presented in teh SERP, even when the ad is direct, and despite the fact that according to our CTR inforamtion it is genrally skipped, it effects the decisions of users that are more prone to chose `Maybe' in comparison to `No' in comparison to the equivalent no ad configuartion. When an indirect marketing ad is present we see a similar behaviour. The suprising result here as that the ads had a similar effect eventhtough their CTR data is different. The direct ads were genralky skipped while the indirect ads were often inspected. Showing that the effect ads have on users is not lmited to users that chose to enter the ad. Merly noticing that its their already introduces a shift in the users` thought process. 


%We continue to inspect SERPs   with a bias towards the inconclusive viewpoint we again see, as expected, that the highest portion of partipants chose the correlating `Maybe' answer for all add configurations. Here too we see a slight decline of the portion of partipants that chose this answer when ads are present. For direct marketing ads, this decrease in divided equally between the two other answer that exhibit a slight increase of 2\% each in comparison to their correlating answer in the no ad configuration. For indirect marketing ads we see a different behaviour with the `Maybe' answer receiving We again see a similar percentage of responses for the `Maybe' and `Yes' responses, this unlike the no marketing and direct marketing ads configuration in which `No' and `Maybe' answers are the ones that receives a similar percentage of the results. This differences are supported by users' examination behaviour. When the ads were direct they users did not enter them and therefore were not greatly influenced by them, but when the ads were indirect, they did choose to enter them and were influenced by them and therefore chose to answer `Yes' more often. Finally we inspect SERPs with a bias towards a negative viewpoint. Here we see that when no ads are present, unlike in the previous viewpoint bias configuration, the result do not correlate to the maximal bias level, with the `Maybe' option receiving the highest portion of answers. This result is explained by peoples general preference to favour positive results. When ads are not present   we see a similar distribution of the `Maybe' and `No' answers, both of tehm are significantly higher than the 14\% poistive responses.  For direct marketing ads we see a similar portion of negative responses For indirect marketing ads we see a high increse of 14\% in the porecentage of negative responses, more than twice the precentege of the `Maybe' response and three tiems the precentage of positive responses. 

%\renewcommand{\arraystretch}{1.35}
%\begin{table}[t]
%\caption{Statistics about the estimated regression weights.}
%\vspace{-2mm}
%\begin{tabular}{|l|c|c|c|c|c| } 
%\hline
%\textbf{Type} & \textbf{Response} &\textbf{\# Non-Zero} &\textbf{Min}&\textbf{Max}\\
%\hline 
%No Ads&Y&9&-1.69 ($^3_M$)&1.15 ($^1_Y$)\\
%\hline 
%No Ads&M&10&0.03 ($^6_N$)&0.89 ($^1_M$)\\
%\hline 
%No Ads&N&13&-1.88 ($^2_Y$)&2.45 ($^8_N$)\\
%\hline
%DM&Y&9&-2.02 ($^3_N$)&1.65 ($^5_Y$)\\
%\hline
%DM&M&7&-0.46 ($^3_N$)&0.81 ($^3_M$)\\
%\hline
%DM&N&11&-1.36 ($^4_Y$)&1.44 ($^5_N$)\\
%\hline
%IM&Y&8&-2.24 ($^4_M$)&1.64 ($^1_S$)\\
%\hline
%IM&M&4&0.10 ($^2_N$)&1.45 ($^6_N$)\\
%\hline
%IM&N&9&-0.41 ($^4_M$) &1.72 ($^2_N$)\\
% \hline
%\end{tabular}
%\label{tab:weight_stats}
%\vspace{-3mm}
%\end{table}


==> Ads paper arXiv/exp.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{0.33\textwidth}
\centering
  \includegraphics[scale=0.33,keepaspectratio]{images/CTR_all.pdf}
  \caption{All marketing Ads.}
  \label{fig:ctr}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
\centering 
 \includegraphics[scale=0.33,keepaspectratio]{images/ctr_direct_marketing.pdf}
  \caption{Direct marketing Ads only.}
  \label{fig:direct}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
  \centering
\includegraphics[scale=0.33,keepaspectratio]{images/ctr_indirect_marketing.pdf}
  \caption{Indirect Marketing Ads only.}
  \label{fig:spon}
\end{subfigure}%
\vspace{-2mm}
\caption{CTR comparison according to maximal bias.}
\label{fig:ctr_ads}
\vspace{-2mm}
\end{figure*}

\begin{table}[t]
\caption{Demographic information of study participants.}
\vspace{-1mm}
\begin{tabular}{ |l|c|c| } 
 \hline
 Age range & 20-74 \\
 \hline
 Average age  & 39 (sd=11) \\
 \hline
 Men & 63\% \\
 \hline
 Women & 37\% \\
 \hline
 With bachelor's degree and above & 61\%\\
 \hline
 No higher education & 39\% \\
 \hline
% average time spent & 5 minutes \\
% \hline
% average links entered & 2.2 links \\
% \hline
% participants that don't have ads & 172 \\
% \hline
% participants that have direct marketing ads & 105 \\
% \hline
% participants that have indirect marketing  ads & 92 \\
 %\hline
\end{tabular}
\label{tab:demographics}
\vspace{-5mm}
\end{table}

\section{Experiment results}
In this section, we will answer our previously defined research questions based on the observations collected from our user study.
Our research questions focus on two important aspects: sponsored content's impact on users' examination behaviour and that on users' decision-making. Section \ref{sec:CTR} will discuss the research question related to users' examination behaviour, and Section \ref{sec:dec} will discuss the research question related to users' decision making. We will also provide summary statistics related to users' self-perception about the effect of sponsored content on their search experience and decision making in Section \ref{sec:exp}.

We filtered out responses from users who did not answer our attention question correctly (81 responses) and responses from users who did not provide any reason supporting their responses (63 responses), which is explicitly required in our instructions. Example of bad reasons provided by users include empty phrase or single word sentences, vague answers such as: ``it provides correct information''. Phrases only describing the treatments or the condition without referring to the effectiveness of the treatment were also removed. 

After filtering, our user study produced 436 valid responses from 436 different participants. Each participant was assigned to a single SERP (i.e., ad configuring-bias level-query condition combination). 
Table \ref{tab:demographics} summarizes the demographic information of the participants, and Table \ref{tab:ads_dist} summarizes the number of responses received for the different settings of each independent variable. In average, each different ad configuration-bias-query triple received 18 observations (std=6).
%summarizes the number of participants that were presented with SERPs for each ad configuration. On average each query-
Participants spent an average of 4.7 minutes on a given SERP (std=3.17) and clicked 2.3 links  (std=1.36) in our study. In total, 992 links were entered by all users, of which 925 (93 \%) were organic results and 67 (7\%) were links to sponsored content. 

\begin{table}[t]
\caption{Levels and descriptive statistics of observations per independent variable}
\vspace{-1mm}
\begin{tabular}{ |c|c|c| } 
\hline
\thead{Independent \\ Variable} & \thead{Levels} & \thead{\#Responses } \\
 \hline
\multirow{3}{*}{
\makecell{Ad \\ Configuration} }& No ads & 157\\
\cline{2-3}
& Direct Marketing &124\\
\cline{2-3}
&Indirect Marketing&155  \\
  \hline
  \hline
\multirow{3}{*}{Query} & Ginkgo-Biloba for  tinnitus&145\\
\cline{2-3}
&Melatonin for jetlag&105\\
\cline{2-3}
&Omega fatty  for treating ADHD & 186\\ 
 \hline
\hline
\multirow{3}{*}{SERP Bias} &Y&125\\
\cline{2-3}
&M&159\\
\cline{2-3}
&N&152\\
\hline
\end{tabular}
\label{tab:ads_dist}
\vspace{-6mm}
\end{table}

\subsection{Impact on Examination 
Behaviour}\label{sec:CTR}
%In this section we will discuss the research questions related to users' examination behaviour.%: 
%\begin{itemize}
%    \item \textbf{RQ1:} Is users' examination behaviour affected by sponsored content on the SERP?
%    \item \textbf{RQ2:} When sponsored content is present, how is users' examination behaviour affected by the organic results on the search page? 
%\end{itemize}

To understand the difference in examination behaviour between the different ad configurations, we examine click-through rate (CTR) of each rank position in the SERP, for the various ads and bias configurations. CTR is defined as the number of times a link was clicked, divided by the number of times it was visible to the users.

Let $r_i$ denote rank position $i$ in a given SERP and $o_i$ denote the rank of $i$th organic result \footnote{An organic result is a search result that is not sponsored} in a SERP. In a SERP without ads, the general documents' ranking and organic results' ranking are the same, therefore $r_i$ equals to $o_i$. When ads are present however, $r_i$ equals to $o_{i-1}$, i.e., the second ranked result is the first organic result and so forth. And lastly, let $CTR(r_i)$ and $CTR(o_i)$ denote the CTR of $i$th ranked document and the $i$th organic result in accordance. 

Figure \ref{fig:ctr} presents CTR over rank positions, for each of the three possible ad configurations. At a high level view of the results, it is evident that the examination behaviour of users is different when ads are present. It is easy to notice that direct marketing ads are generally ignored by users and indirect marketing ads receive significantly less clicks than organic results at the same rank position. 

%We first examine the CTR of the first ranked result, i.e., $CTR(r_1)$. Unlike entries in rank 2 and afterwards, which can only belong to organic content, the first ranked result can be either an ad or an organic result, depending on the ad configuration of the SERP.

As can be seen from the figure,
when ads are not presented (i.e., the first ranked position is organic result), the first position receives the most attention from users, with a CTR at around 0.58. This is in comparison to a CTR of 0.37 when the first ranked result is an indirect marketing ad and only 0.07 when the first ranked result is a  direct marketing ad.
A one-way ANOVA test comparing $CTR(r_1)$ among all three ad configurations revealed that this difference is statistically significant (F(2,433)=46, p<0.01). A further post-hoc Tukey’s HSD test for multiple comparisons revealed that the mean value of each pair of configurations was significant as well, meaning that there is a significant difference not only between $CTR(r_1)$ in SERPs with no ads compared to SERPs with ads, but also between the two different ad configurations, with p < 0.01 for all comparisons. 

%A difference to which we will soon investigate.
%The , $r_2$, correlates to $o_2$ for SERPs without ads and to $o_1$ for SERPs with ads. 
In the second ranked position, we see that for ad-free SERPs the CTR declines from 0.58 to 0.4. In contrast, the exhibited examination behaviour when ads were presented shows an increased CTR on the second position from 0.37 to 0.56 for SERPs with indirect marketing ads and from 0.07 to 0.55 for SERPs with direct marketing ads, values similar to that of $r_1$ in the no ad configuration. This suggests the first organic result receives similar attention in all ad configurations. A one-way ANOVA test of $CTR(r_2)$ between the three ad configurations again showed a statistically significant difference (F(2,433)=46, p<0.02). This time the post-hoc Tukey’s HSD test revealed a significant difference only between the `No Ads'  and each ad configuration, but not between the two ad configurations.
This clearly demonstrates that, despite the ad's position advantage, participants showed a clear preference towards organic results; or in other words, a strong tendency to skip the ads.

%groups were not statistically significant as expected by the similar values (p>0.8). %Comparing the CTR values according to organic result rankings, we see very similar values between $CTR(o_1)$ for all three ad configurations (0.58,0.55,0.56). Showing that first organic results received similar attention from users in all configurations. 

%We continue to examine $r_3$, where we see a clear drop in CTR for all three ad configurations. With the CTR declining to 0.27 when no ads are present, and to 0.44 and 0.39 for direct and indirect ad configurations respectively. A one-way ANOVA test of $CTR(r_2)$ between the three configurations again showed a statistically significant difference (F(2,433)=5.12, p<0.01). The post-hoc Tukey's HSD test revealed a strong significance level between the `No Ads' and `Direct Marketing Ads' configurations (p<0.01) and a weak significance level between the `No Ads' and the `Indirect Marketing Ads' configurations (p<0.07). No significant difference was found between the two ad configurations (p>0.5). We again compared the CTR according to the organic results' ranking $CTR(o_2)$ = (0.41,0.44,0.39), which again show no statistically significant difference. Again demonstrating that similar organic result ranking receives similar attention from users. 

%As the position of documents continues to decrease the differences between the various ad configurations as can be seen in the figure. Specifically, from $r_4$ and afterwards, ANOVA analysis did not reveal a statistically significant difference between any of the three configurations.

%each ad configuration. The CTR between the two ad groups were no statistically significant as expected by the similar values. 
%Comparing the CTR values according to organic results ranking we indeed very similar values between $CTR(o_1)$ for all three ad configuration (0.58,0.55,0.56). Showing that first organic results received similar attention from user in all configurations.


%Although the CTR in these group is still higher than that of the no ads configuration. (F(2,433)=5.12, p<0.01).
%$r_3$ correlates to $o_2$ for two ad groups.
%The CTR of $r_3$ for the for the direct and indirect ad groups (0.44, 0.38)  are similar to the CTR  of $r_2$ for the no ads group (0.4) but different that the CTR of $r_3$ for the no ads group (0.26)


%We conducted a one way ANOVA analysis between organic results of these ranks between the three configuration groups. A comparison between $o_1$ for all groups would compare $CTR(r_1)$ for the no ads groups and $CTR(r_2)$ for the two ads configuration groups. The analysis did not reveal a significant result for any of the groups. Showing that when it comes to organic results the examination behaviour between all groups is similar to each other. 


%As can be seen from the graph and the analysis above, often times, the $CTR(r_i)$ for the two ad groups correlates to $CTR(r_{i-1}$ in the `No ad' group, or in other words $o_i$. To confirm this observation we  





%A further two way comparison ttest between each of the two subgroup also did not produce statistical significant results, showing that the first organic link in all configurations receive similar attention. 

%To compare the effect of the ad configuration on the CTR of the first link we 

%It appears that users tend to skip the ad and progress to the first organic result. Once the ad is skipped they maintain their preference to higher ranked results. 

%This is especially noticeable with direct marketing ads where the ad is clicked for only 10\% of times. 
%Although small, this numbers is still significantly larger than the average CTR for ads in the health industry which stands at 3.37\%


%\begin{table}[t]
%\caption{ANOVA results for comparison between CTR's of different ranks and ad configurations}
%\vspace{-1mm}
%\begin{tabular}{ |c|c|c|c| } 
%\hline
%\thead{No Ads} & \thead{Direct \\ Marketing \\ Ads} & \thead{Indirect \\ Marketing \\ Ads } &\thead{ANOVA \\ Result} \\
%\hline
%$CTR(r_1)$&$CTR(r_1)$&$CTR(r_1)$ &F(2,433)=46, p<0.01\\
%$CTR(r_2)$&$CTR(r_2)$&$CTR(r_2)$ &F(2,433)=4.48, p<0.02)\\
%$CTR(r_3)$&$CTR(r_3)$&$CTR(r_3)$ &F(2,433)=5.12, p<0.01)\\
%$CTR(r_i, i > 3)$&$CTR(r_i, i > 3)$&$CTR(r_i, i > 3)$ &Insignificant\\
%$CTR(o_i)$&$CTR(o_i)$&$CTR(o_i)$ & Insignificant\\
%\hline
%\end{tabular}
%\label{tab:ads_dist}
%\vspace{-2mm}
%\end{table}


%We now go back to the difference between the CTR of the first position in SERPs with direct marketing ads versus SERPs with indirect marketing ads.
%As demonstrated by the statistical analysis and also evident in the graphs,
%As evident in the figures and supported by previous statistical analysis, while the $CTR(r_1)$  for  SERPs with indirect marketing ads is lower than the $CTR(r_1)$ for SERPs with no ads, it is also significantly higher when compared to $CTR(r_1)$ for SERPs with direct marketing ads.
%To invesitge this diffrence with divised the 
%A further inspection of graph Although all results were significant it can clearly be seen that this difference is more significant for direct marketing ads than in indirect marketing content ads, in fact for indirect marketing ads the CTR of first rank is only slightly lower than that of the third link and is higher than that of the forth link. 

To better understand the effect of the different ad configurations on users' examination behaviour,
%To investigate the difference between the CTR of the first position in SERPs with direct marketing ads versus that in SERPs with indirect marketing ads
we further decompose the CTR of the two ad configurations according to the maximal a priori bias level in the SERP, as detailed in Table \ref{tab:configs}. 
Figures \ref{fig:direct} and \ref{fig:spon} show the CTR distribution by maximal bias level for SERPs with direct and indirect marketing ads.

As can be observed in Figure \ref{fig:direct}, for SERPs with direct marketing ads, a similar examination behaviour is exhibited across all bias levels: The CTR of the first position is generally very low, while the CTR of the second position receives significantly higher attention. %We then observe a drop in the CTR of the third link in comparison to second. A closer inspection revels that for the `N' configuration the second and third entries received similar attention with $CTR(r_2)=0.58$ and $CTR(r_3)=0.54$, indicating that in this configuration partipants gave the first two organic results similar attention.Although this drop is not as high as that observed in the no ads configuration, with a drop of 0.15 for  'Y' SERPs, 0.13 for `M' and only 0.04 for `N'. 


%Figure \ref{fig:direct} shows that in SERPs with direct marketing ads CTR of the first position is generally very low for all bias levels. The second position received significantly higher attention, a behaviour which again repeats for all bias levels.
%We continue to similar CTR values as the position of results in the SERP decreases, between all three bias configuration groups. %Indeed a one way ANOVA analysis of the the $CTR(r_i)$ between the three bias levels did not find any statistically significant differences.

But surprisingly, this is not the case in SERPs with indirect marketing ads. As shown in Figure \ref{fig:spon}, participants' behaviour is not uniform across all bias levels. The curve for the negative bias configuration (i.e., `N') behaves quite similarly to that of the curves presented in Figure  \ref{fig:direct}, with a very low CTR for $r_1$ (0.18) that jumps to a very high CTR (0.68) for $r_2 / o_1$, and declines to 0.37 for $r_3/o_2$.
%and then continuous to generally decline as the position ranking of document decreases. 
This suggests that when the bias of the SERP is negative the ads are generally ignored by the users. When we inspected the other two bias configurations, however, we encountered different observations. In these configurations, we do not see the behaviour exhibited in the direct marketing ad setting. 
%(i.e., a tendency to generally skip the ads); 
And on the other hand, the behaviour is not similar to that exhibited by the no ad configuration either, where $CTR(r_1)$ is significantly higher than $CTR(r_2)$ and on wards. 
%. What we are seeing in fact, is a similar CTR between the first 
In SERPs with positive bias (i.e., `Y'), we see that the CTRs for the first three rank positions are similar to each other at around 0.4. The significant decline only begins at $r_4/o_3$, which drops to 0.25. In SERPs with inconclusive bias (i.e., `M'), we see a similar CTR of the two highest rank positions of 0.51 and 0.54, followed by a decrease to 0.37 for $r_3/o_2$. 




We believe the reason for these observations stems from the level of contrast between viewpoints of the organic and sponsored content. Bear in mind that indirect marketing ads are essentially web pages that present content supporting the effectiveness of the treatment. This supporting opinion is evident not only by reading the content but also from the title and snippet of the presented results in the SERP.
%, as it is for the other web pages as well. 
When the SERP's bias level is towards the negative viewpoint, the opinion in the ad is strongly contradicted by the organic results, i.e., the contrast between the ad's viewpoint and the bias of the organic result is high.
The participants can notice this fact, skip the ad, and proceed to click on the organic results.
However, when the contrast is
%between the content presented in the ad and the viewpoint presented by the organic results 
not high, participants are more prone to inspect the content of the ad. 
%They are still aware, however, that the content is sponsored as it is explicitly highlighted as ``Ads'' and continue to inspect further organic content before reaching a conclusion.  
We hypothesize that because the indirect marking ads typically have rich content, e.g., its title and abstract often contain professional or medical terms, when the contrast level is low, the users tend to reduce their negativity towards sponsored content and are more willing to open the link for further investigation. Please note in our setting one MTurk worker can only encounter one SERP configuration and thus they were not aware of the different biases manufactured in our study. As we will present in Section \ref{sec:exp}, interestingly, although almost all our participants reported they were not affected by the presence of sponsored content, their examination behaviors already differed conditioned on what types of sponsored content were presented.


Our observations lead to mostly reject hypothesis H1: Although in some cases, users do skip ads and prefer higher ranked organic results, there is still a non-negligible portion of cases where the users inspect the ads. 

%They do not rely solely on the sponsored content and wish to back up their decision by inspecting organic results as well. 

%Perhaps because they are still aware to the possible bias in sponsored content. 


%TTEST results 
%A versus S and organic restuls 
%summarize answer to 2 research  questions 


\subsection{Impact on Decision-Making}\label{sec:dec}

\begin{table}
\caption{Participants' responses absolute and percentages values, grouped by ads-bias configurations.}
\vspace{-1mm}
 \begin{tabular}{|c|c|c|c|}
\cline{2-4}
\multicolumn{1}{c|}{}  & \textbf{Yes} & \textbf{Maybe} &\textbf{No}\\
\hline
\textbf{Y}&28(0.52)&14(0.26)&12(0.22)\\
\hline
\textbf{DY}&15(0.45)&14(0.42)&4(0.12)\\
\hline
\textbf{IY}&14(0.41)&15(0.44)&5(0.15)\\
\hline
\hline
\textbf{M}&12(0.24)&25(0.50)&13(0.26)\\
\hline
\textbf{DM}&11(0.26)&20(0.47)&12(0.28)\\
\hline
\textbf{IM}&25(0.39)&27(0.42)&12(0.19)\\
\hline
\hline
\textbf{N}&7(0.14)&22(0.44)&21(0.42)\\
\hline
\textbf{DN}&10(0.22)&16(0.35)&20(0.43)\\
\hline
\textbf{IN}&9(0.17)&14(0.27)&29(0.56)\\ 
\hline
\end{tabular}
\label{tab:user_conf}
\vspace{-2mm}
\end{table}

\begin{table}
\caption{T-Tests comparisons between the different answers for all ad-bias configurations.  \checkmark\ \checkmark stands for $p< 0.01$,  \checkmark  for $p < 0.05$, and $\times$ for $p \geq 0.05$.}
\vspace{-1mm}
 \begin{tabular}{|c|c|c|c|}
\cline{2-4}
\multicolumn{1}{c|}{}&\thead{Yes-\\Maybe}&\thead{Yes-\\No}&\thead{Maybe-\\No}\\
\hline
\textbf{Y}&\checkmark \checkmark&\checkmark \checkmark&$\times$\\
\hline
\textbf{DY}&$\times$&\checkmark \checkmark&\checkmark \checkmark\\
\hline
\textbf{IY}&$\times$&\checkmark \checkmark&\checkmark \checkmark\\
\hline
\hline
\textbf{M}&\checkmark \checkmark&$\times$&\checkmark \checkmark\\
\hline
\textbf{DM}&\checkmark \checkmark&$\times$&\checkmark \checkmark\\
\hline
\textbf{IM}&$\times$&\checkmark \checkmark&\checkmark \checkmark\\
\hline
\hline
\textbf{N}&\checkmark \checkmark&\checkmark \checkmark&$\times$\\
\hline
\textbf{DN}&\checkmark &\checkmark \checkmark&\checkmark \\
\hline
\textbf{IN}&\checkmark &\checkmark \checkmark&\checkmark \checkmark\\
\hline

\end{tabular}
\label{tab:ttest}
\vspace{-3mm}
\end{table}


We now focus on the research question about users' decision-making process.
%\begin{itemize}
%    \item \textbf{RQ3:} Is user decision-making affected by sponsored content on the search results page?
%    \item \textbf{RQ4:} When sponsored content is present, how is  user decision-making affected by the organic results on the search page? 
%    %\item \textbf{RQ4:} Is the attitude if users' towards sponsored content effected by the organic results in the search page? 
%\end{itemize}

Table \ref{tab:user_conf} shows the distribution of participants' responses grouped by ad configuration and the maximal level of posterior bias computed by Eq \eqref{eq:bias}.
The posterior bias level is computed in a similar way as the priori bias level, 
%with only one difference. Instead of estimating a position's CTR using its rank, we 
but by using the actual CTR observed in our study data: $P_c(i) = CTR(r_i)$. As can be seen in Table \ref{tab:configs}, while the absolute values of the posterior and priori bias levels are slightly different, the order among viewpoint bias remained the same. This means that 
%our initial assumption about the correlation between rank position and users' click probability was confirmed by our collected data and 
our participants behaved as expected according to our existing knowledge on position bias \cite{craswell2008experimental}. 

Each row in Table \ref{tab:user_conf} corresponds to an ad configuration and a bias level. The rows noted by a single letter (`Y', `M', `N') describe the response distribution across different bias levels of ad-free SERPs, and the rows marked by two letters describe users' response distribution across different bias levels for SERPs with either direct (D) or indirect (I) marketing ads. 
The columns represent the number of responses  along with the percentage of responses in parenthesis:  ``Yes'' for a positive response, ``Maybe'' for an inconclusive response, and ``No'' for a negative response. Out of 436 responses, only 10 were `No Sure'. For clarity of presentation, they were therefore discarded from the analysis.
Table \ref{tab:ttest} summarizes the t-test results of the portion of results each answer received for the different ad-bias configurations. 

From the results we can see that in the no ads configurations, there is a correlation between the maximal bias level and the most popular response, which aligns with previous work on position bias.
This is very evident for the ``Y'' and ``M'' bias levels and less evident for the ``N'' bias level. We can also see that for each bias configuration a different user behaviour pattern is exhibited in at least one of the ad configurations.

For indirect marketing ads, we can observe ads' influence in all bias levels, with the direction of the influence depending on the SERP`s bias level. When the viewpoint bias of the SERP is either positive or inconclusive (i.e. rows ``IY'' and ``IM''), we observe a decrease in the portion of negative responses in both configurations. For the ``IY'' configuration, we then observe an increase in the portion of ``Maybe'' responses; and for the ``IM'' configuration,  an increase of the ``Yes'' responses. 
We also observe that in both configurations the ``Maybe'' and ``Yes'' responses receive a similar portion of the answers. These observations coincide with the CTR data for these configurations. For the ``IM'' configuration, we observed that the first 2 positions received similar attention from partipants. These positions represent an ad and an inconclusive viewpoint organic result. For the ``IY'' configuration, we observed that the first 3 positions received similar attention. These positions represent an ad, a positive viewpoint organic result, and another organic result that can belong to either viewpoint. In these configurations, when indirect marketing ads are present, users were exposed to a wider viewpoint distribution in comparison to the corresponding no ads configuration, which in turn affected their decisions. 
%When the viewpoint bias of the SERP is either positive or inconclusive (i.e. rows ``IY'' and ``IM'') the ads introduce positive bias. A t-test comparison revealed that in the ``IY'' configuration the ``Maybe'' answer received a significantly higher portion of the responses compared to the `Y' configuration (t(86)=1.78, p=0.039); and that in the ``IM'' configuration the ``Yes'' answer received significantly more responses  in comparison to the ``M'' configuration (t(112)=1.71, p=0.04).
%These observations coincides with the CTR data that showed partipants did tend to click the ads for configurations ``IY'' and ``IM''. When the SERP is biased towards a negative viewpoint, the ads introduce negative bias. This is despite the fact that according to our CTR data, in this setting partipants tended to skip the ad. A t-test comparison revealed that in the ``IN'' configuration the ``Maybe'' answer received a significantly lower portion of the responses compared to the `Y' configuration (t(100)=1.81, p=0.036). 

Direct marketing ads are rarely inspected according to our CTR data. Nevertheless they still affected users' decisions, although in a more subtle manner than indirect marketing ads. The effect, when exists, is always towards the positive side. 
For the ``DY'' configuration we observe a shift from ``No'' to ``Maybe''.
%A t-test comparison revealed a weakly significant difference in the portion of ``Amyber'' response in the ``DY'' configuration in comparison to the ``M'' configuration (t(112.0)=1.44, p=0.07).  
We observe no significant difference for the ``DM'' configuration; and for the ``DN'' configuration we see a shift from ``Maybe'' to ``Yes''. 
%although no statistically significant difference was found between the ``DN'' and ``N'' configuration for any of the answers.


%Next we will examine these results according to the maximal bias level in the SERP.

%When the maximal bias level is towards the positive viewpoint, we see that in both the ``DY'' and ``IY'' configurations there is a shift from the ``No'' answer to the ``Maybe'' answer. Causing the ``Maybe'' option to receive a significantly higher portion of the responses comparing to the `Y' configuration. This difference is weakly significant for ``DY'' versus `Y' (t(85.0)=1.6, p=0.056), and strongly significant for ``IY'' versus`Y' (t(86.0)=1.78, p=0.039). In fact, in this bias level when ads are present, the ``Yes'' and ``Maybe'' answers receive a similar portion of responses; but without ads, the ``Yes'' answer receives a significantly higher percentage than both ``Maybe'' and ``No''.

%When the maximal bias level of SERPs is towards the inconclusive viewpoint, we see that indirect marketing ads introduce positive bias, with a significantly higher portion of ``Yes'' responses for ``IM'' in comparison to both `M' (t(112.0)=1.71, p=0.04) and ``DM'' (t(112.0)=1.44, p=0.07). Here, the portion of participants who answered ``Yes'' is similar to that of participants who answered ``Maybe''. Unlike the `M' and `IM' configurations, where the ``Maybe'' response is significantly higher than that of either ``Yes'' or ``No''.

%When the maximal bias level of SERPs is towards the negative viewpoint,we see a clear negative bias invoked by indirect marketing ads, with a higher portion of ``No'' answers for ``IY'' in comparison to ``Y'' and a significantly lower portion of ``Maybe'' responses (t(100.0)=1.815, p=0.036). We also observe a slight shift from ``Maybe'' to ``Yes'' for direct marketing ads. Although this change does not result in a significant difference between the portion of responses between the ``N'' and ``DN'' configurations, for any of the three possible answers. 

%We now summarize our main findings. Firstly, in the no ads configurations, we see that there is correlation between the maximal bias level and the most popular response, which aligns with previous work on position bias. This is very evident for the ``Y'' and ``M'' bias levels and less evident for the ``N'' bias level. %This might be explained by users misinterpreting the negative content in an overly optimistic manner. 
 
%The manner of this effect depends on the type of the ads as well as on the level of bias in the SERP.
%For indirect marketing ads we see that the bias invoked by the ad depends on the position bias of the organic results presented in the SERP. 
%For the ``IY'' and ``IM'' configurations, where there is low to no contrast between the viewpoint presented in the ad and in the organic results, we see a stronger inclination to take the viewpoint of the ad under consideration. This is also supported by the CTR data which showed that under these configurations the ads are inspected quite often. However, when the organic results strongly disagree with the ad, it elicits a strong negative bias, even when users did not enter the ads.%Direct marketing ads are rarely inspected according to our CTR data. Nevertheless they still affect users' decisions, although in a more subtle manner. In this configuration, the effect is always towards the positive side. 

We hypothesize that the difference between partipants' reaction to the two ad types is due to the difference between the manner in which these two  types support the treatment`s effectiveness. Direct marketing ads offer the treatment for sale but do not explicitly support its effectiveness. Indirect marketing ads explicitly support the treatment's effectiveness by eagerly announcing its helpful qualities already in the title and snippet of the ad. Indirect marketing, therefore, elicits stronger sentiment, either positive or negative depending on the organic results presented in the SERP. 

%Indirect marketing ads support the treatment`s effectiveness. as opposed to the implicit nature in which direct marketing ads support it by offering it for sale without 
 %by eagerly announcing its effectiveness already in the title of and snippet of the ads
 % supporting or even discussing its effectiveness.

%When the maximal bias level is towards the positive viewpoint and no ads are present, the ``Yes'' answer is chosen by most participants at a percentage which is significantly higher than that of participants that chose either ``Maybe'' or ``No''. The percentages of participants that chose `Maybe' or `No', however are not  significantly different from each other.A different behaviour is exhibited when ads are present. In both the direct and indirect marketing ad configurations, we see a similar portion of participants choosing either ``Yes'' or ``Maybe'', while a significantly lower portion of the participants chose the `No' answer. These results indicate that in positively biased SERPs, where the viewpoint presented by the ads aligns with the viewpoint ranking bias expressed in the SERP, participants that consumed negative viewpoint content were effected not only by the ranking bias of the SERP in general but also by the ads and opted for a ``Maybe'' response more frequently.  And this occurred regardless of whether or not they consumed the content in the ad. 


%When the maximal bias level of SERPs is towards the inconclusive viewpoint, we see that when no ads are present the correlating `Maybe' response received the highest portion of answers. A percentage that is  again significantly higher the that  of responses received for the remaining two options ``Yes'' and ``No'', which were, as in the positive viewpoint with no ads, similar to each other. When examining the ads configurations for this bias setting, we see different behaviours between the direct and indirect marketing ads configurations. When direct marketing ads are present, we see a similar behaviour to that of the no ads configuration. However, with the indirect marketing ads, we see that the ``Yes'' and ``Maybe'' responses receive a similar portion of responses,  while the ``No'' response receives a significantly lower percentage of responses.We hypothesize that since the viewpoint of the SERP was not definite, participants were not effected by direct marketing ads. This might be due to the fact that its opinion regarding the treatment effectiveness is very implicit. They were however affected by the indirect marketing ads where we see a lower percentage of negative answers and a higher percentage of positive answers.
%We see a general shift towards more positive answers. 
%We hypothesise that participants that were exposed to the ad in addition to negative content were more likely to chose the `'Maybe'' answer and participants that exposed to the ad in addition to inconclusive results were more prone to choose ``Yes''.


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{images/heatmap_C_1_by_answer2.pdf}
\vspace{-3mm}
\caption{HeatMap for logistic regression learnt feature weights.}
\label{fig:HeatMap}
\vspace{-3mm}
\end{figure}
%\subsubsection{Correlation Between Behaviour and Decision Making}
%Sections \ref{sec:CTR} and \ref{sec:dec} inspected the effect of ads on examination and decision making in relation to ad configuration and SERP bias levels. 
To better understand the connection between ads and users' decisions, we also examine the effect of ads on the correlation between users' examination behaviour and their decisions. To achieve so, we trained a set of multi-class logistic regression classifiers and analyzed their learnt feature weights. These classifiers were fitted to predict a user's response given the SERP presented to her based on her observed clicks.
A model was trained for each of the three possible ad configurations independently. 
%The feature vectors inserted to each model represented data collected only from experiments assigned to that configuration. Each feature vector was constructed from a set of 
Binary features in the form of $f_i^l=\{0,1\}$ were constructed to encode users' clicks, where $i$ denotes the position of a document and $l$ denotes the viewpoint label (`Y', `M' or `N') or the ad configuration (`D' or `I') of that document. $f^i_l=1$ if the document at position $i$ with label $l$ was clicked, and 0 otherwise. For example $f^1_D=1$ means that in one experiment the user clicked on the direct marketing ad at position 1.
%A logistic regression model fits a set of weights for each feature. The features` weights correlate to their impact on the classification, either positively or negatively, according to the sign. For multi-class regression, a weight vector is constructed for each possible class. 
%We denote by $w_r^i$ the weight assigned by the model to feature $f_r^i$. 
Figure \ref{fig:HeatMap} shows a heat-map of the learnt weights. We used  $\ell_1$ regularization for feature selection purposes, to help the classifiers learn the most significant features. The X axis denotes the features $f^i_l$ and the Y axis denotes the ad configuration and the user's response class (comma separated) under which the model was trained.


%For participants who answered  ``Yes'',  we can observe that in all ad configurations, positive weights were assigned only to positions with either ads or positively labeled results. We can also observe strong effect of the first ranked result for both no ads and indirect marketing ads configurations, while with direct marketing ads the most influential positions are the ones ranked from 2 to 5, which usually correlates to the first result viewport. This reaffirms our previous observation that indirect marketing ads can influence participants' decision when their content is consumed. 
%For all ad settings we're seeing that positively labeled results had only positive weights while negative and inconclusive entries had only negative weight, e.g being a counter indication of the user selecting a positive response.

%For participants who answered ``Maybe'', we  observe a wider exploration pattern and stronger tendency to scroll down to the lower part of the SERP. We can also observe influence from all types of entries, with positive weights assigned to positions with positive, inconclusive and negative labels, in all ad configurations.  In particular, for the no ads configuration, as expected, clicking on the first result when labeled as inconclusive is a strong indicator about  the ``Maybe'' response. In both ad configurations, however, we observe the ad does not affect participants' decisions. We can draw from this that participants that answered ``Maybe'' were less affected by sponsored content for both its types. 

%For participants who answered ``No'', we can find that in all ad configurations, positive weights were assigned only to positions with negative  results.  We can also observe that while direct marketing ads had no affect on the users, consuming indirect marketing ads had a negative impact on choosing a negative response. Again showing that indirect marketing ads can affect users' decisions. 


Inspecting the heat map, we can observe a general correlation between the viewpoint of users' inspected content and their decision, validating our experimental methodology.
For the models predicting ``Yes'' and ``No'' answers, only correlating viewpoints (i.e  features of the form $f^1_Y$ for ``Yes'' and $f^1_N$ for ``No'' ) received a positive weight, in all ad configurations. For the models predicting ``Maybe'' we observe positive influence of entries from all three viewpoints, however no influence from either ad type. 
We can also observe that consuming the content of indirect marketing ads influences users to select a positive response, with ($f^1_I$) receiving a positive weight in the model ``Indirect Marketing, Yes'' and a negative weight in the model  ``Indirect Marketing, No''. This suggests that when consumed, indirect marketing ads introduce positive bias to the decision making process. We do not observe any correlation between clicking on direct marketing ads and the various responses, as expected given their low CTR. Bear in mind that the regression only inspected the effect of positions that were clicked and cannot infer the effect of consuming the ads' title and snippet content without clicking on the link. 

%In the model predicting  ``Yes'' , only features of the form $f^i_Y$ receive a positive weight, in the model predicting  ``No'', only features of the form $f^i_N$ receive a positive weight. For the model predicting  ``Maybe'' we see positive weights from all three result labels. 
 

%The main conclusions that we can draw from the regression results are that first of all, as expected, there is correlation between the viewpoint of user inspected content and their decision, especially in participants who provided definite answers (e.g ``Yes'' or ``No''). We can also observe that consuming the content of indirect marketing ads influences users to select a positive response. We do not find such behaviour under direct marketing ads. However, bear in mind that the regression only inspected the effect of positions that were clicked on and cannot inspect the effect of consuming the ads title and snippet values. 

%Table \ref{tab:weight_stats} summarized the main statistics of each model's learnt weights, denoting the number of non zero weights as well as the min and max values along with their corresponding response classes. 

%As can be seen from both Figure \ref{fig:HeatMap} and Table \ref{tab:weight_stats}, the learnt weight vectors are sparse.%, expect for the model of a negative response for ad-free SREPs, all weight vectors contain ten or less non-zero weights. Most of the strong response predictors are located at the higher ranked position. For SERPs that contain ads, we can clearly see stronger influence of organic results in comparison to ads. For SERPs with direct marketing ads, clicking on the ad was a negative indicator for selecting a negative response (weight = -1.3). And on the other hand, for SERPs containing indirect marketing ads, the model recognized clicking on the ad as a strong indicator of a positive response (weight = 1.63).



We are now ready to answer our research questions whether sponsored content affects users' decision making. And our answer is affirmative. We therefore also reject H2 which hypothesised that ads do not affect users decision making. 
As our results indicate, sponsored content can introduce either positive or negative bias, depending on the type of the ad as well as on the bias presented by the organic results. 
%When the SERP is biased towards an inconclusive viewpoint, we see that direct marketing ads do not affect the users at all, as opposed to indirect marketing ads that introduce a positive bias. When the SERP is biased towards a negative viewpoint, however, both direct and indirect marketing ads introduce additional negative bias, with a higher level of bias introduced by indirect marketing ads (meaning the user is more likely to respond `No' in their answer). Considering the fact that according to Section \ref{sec:CTR} participants did not click on the ad in these configurations of SERPs, and therefore they did not consume the ads' content (at most the displayed title and abstract in the SERP). This observation suggested an innate preexisting bias towards ads in users in general.  




\subsection{Impact on Search Experience}\label{sec:exp}

%\begin{figure*}[h]
%\centering
%\begin{subfigure}{0.48\linewidth}
%\centering 
% \includegraphics[scale=0.45,keepaspectratio]{images/ad_exp_effect_py.pdf%}
%  \label{figure:direct}
%  \caption{Ads Effect on Users Experience}
%\end{subfigure}
%\begin{subfigure}{0.45\linewidth}
%  \centering
%\includegraphics[scale=0.45,keepaspectratio]{images/ad_dec_effect_all_py.pdf}
%  \label{fig:spon}
%  \caption{Ads Effect on Users Decision Making}
%\end{subfigure}%
%\caption{CTR comparison according to maximal bias}
%\label{fig:user_reports}
%\hnote{Can we put these two bar plots into one figure?}
%\end{figure*}

Participants whose SERP contained ads were requested to rate the ads' effect on their search experience and their decision-making process. The distributions of participants' responses for both questions are reported in Figure \ref{fig:user_reports}. 
The vast majority of participants reported that the ad did not affect either their search experience or their decision-making. There was no significant difference between the two ads configurations.
%70\% of participants reported that the ad had no effect on their search experience, 13\% reported a minor negative effect and 11\% reported a minor positive effect, and about 5\% of participants reported major effect on their search experience (2\% negative and 3.4 \% positive).  

%When it comes to decision-making, 81.5\% of participants reported that the ads did not effect their decision, 5\% reported a  minor negative effect and 7.5\% reported a minor positive effect. About 5\% reported a major effect (1.3\% negative and 4.7 \% positive).
69 participants provided comments about the effect of the ad on their experience. Most of the participants (58) comments were neutral, noting that they did not mind or notice the ad in the experiments, and they said they tended to ignore ads in general.
For example: 
``\textit{I ignored the ad that I saw and skipped down to the first non-ad link.}'',
 and ``\textit{Honestly, I don't look at ads. I never open them when I'm researching.}'' 
Some participants expressed dissatisfaction in their comments. For example:
``\textit{Intrusive and annoying.  The world is one big ad.}''. 
And some admitted the negative bias that ads invoke in them, for example: ``\textit{I notice them, but automatically disregard them as unreliable.}'',  ``\textit{I usually ignore ads, I don't trust them.}'', and `` \textit{I generally skip over the ads when looking for actual information.  I'm not going to go with a paid ad for research purposes.}''.
Only one participant had positive comments about the ads noting that they were informative and relevant to the search.  

To summarize, the participants' responses and comments indicate that the majority of them perceived themselves as unaffected by ads. However, the results presented in the previous sections suggested that oftentimes this is not the case, as both their examination and decision-making are affected by the sponsored content presented in the SERPs. 

%However, the results presented in the previous sections about examination behaviour and response distribution reveal that this not the always case. T
 
%their examination behaviour and decision making data, this is not the case. 
%However our results indicate that 
%and users are influenced by the existence of ads. 
%Although users perceive their decision as independent and not effected by the existence of ads, 
%Although users are aware of ads and the negative sentiment they arise them 
%These results correlate to the data about participant's behaviour and decision making.  

\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth,scale=0.2,keepaspectratio]{images/ads_effect.pdf}
\vspace{-6mm}
\caption{Ads effect on users' experience.}
\label{fig:user_reports}
\vspace{-6mm}
\end{figure}

==> Ads paper arXiv/intro.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.35,keepaspectratio]{images/adhd_natural.pdf}
\caption{Results for the query: `Natural remedies for adhd'. }
\label{fig:example}
\vspace{-3mm}
\end{figure}

\section{Introduction}

%\begin{figure*}[h]
%\centering
%\begin{subfigure}{0.4\linewidth}
%\centering
%\includegraphics[scale=0.45,left,keepaspectratio]{images/how to treat adhd in kids croped.pdf}
%  \label{figure:treat1}
%\end{subfigure}
%\begin{subfigure}{0.4\linewidth}
%  \centering
%\includegraphics[scale=0.45,keepaspectratio]{images/Natural Remedies for ADHD croped.pdf}
%  \label{fig:treat2}
%\end{subfigure}%
%\caption{Results by Google for ADHD treatment queries}
%\label{fig:example}
%\end{figure*}


%Search engines queries represent various types of information needs. Some queries are simple like navigational queries and search of simple factual information like train schedules or the weather.
Search engines are a gateway to information, which help users make informed decisions in various aspects of their lives. This includes decisions about their health ~\cite{PEW}.
Users trust that search engines will present them with accurate and reliable results~\cite{PEW_trust}. However, this trust can make them susceptible to biases in the search results: 
whether it is the general and often positive bias of the presented results
~\cite{white2014content, white2013beliefs}; or the users' own tendency to inspect mostly the top results on the page 
~\cite{joachims2017accurately,keane2008people,o2006modeling,pan2007google}. In the health domain in particular, it has been shown that users are mainly susceptible to positive bias when researching medically related topics  ~\cite{allam2014impact,pogacar2017positive,white2013beliefs,hashavit2021understanding}. This problem can be exacerbated when financial and marketing influences come into play, if, for example, people count on natural remedies or vitamins as an alternative to professional medical treatment or vaccinations. This is a concerning phenomenon especially now during the COVID pandemic, when consuming inaccurate medical information can be life threatening.

%Research shows that user's attitude is effected by the results presented to them in search eniges. Theya re effected by bias in search engines and can be skewed as aresult of the reaults presented to the in the SERP. 
%They trust them so much that they rarely interact with results past the first result page. Position bias,,,

On the other hand, search engines are also a powerful advertising platform since the advertisers can connect their content to relevant queries, thus specifically targeting relevant audiences~\cite{varian2006economics}. Ads are usually presented at the top of the search result page (SERP), ensuring that they are visible to users.
Search engine advertising has become very common and users are accustomed to encounter ads in their SERP. As a result, they sometimes develop a tendency to disregard the ads; skipping over them as if they do not exist, a phenomenon often referred to as banner blindness~\cite{li2019user,foulds2021investigating,burke2005high}.
Nevertheless, marketing research shows search engine advertising is an effective tool advancing various consumer metrics, such as brand awareness and brand consumption, even among users who do not click on the ads \cite{searchAdsEffect}.

In this work we focus on healthcare related search engine advertising. 
%The healthcare and pharmaceutical industry is a large consumer of digital advertising, investing billions of dollars a year advertising in online platforms. In the US, the healthcare and pharmaceutical digital advertising spending is evaluated at about 7\% of all digital ad spending~\cite{healthStats}.
As sponsored content can introduce additional bias to the presented results, it can present a potential issue when the search process is part of a user's decision-making process in health-related problems. 
%Although during the COVID pandemic search engines have exerted immense efforts to prevent misinformation and to promote accurate content~\cite{covcc}, other, perhaps less ominous, conditions do not enjoy the same protection~\cite{cai2021using}.
Take for example a parent who has a child with attention deficit hyperactive disorder (ADHD)
%that wishes to learn about the available options to help their child.
and wishes to explore options of natural-based remedies for treatment of ADHD.
The parent starts their research with their trusted search engine. Figure  \ref{fig:example} shows the top of the result page for the query ``natural remedies for ADHD''.
%produced by a popular commercial search engine. 
%two  queries a parent might start their research with: `How to treat ADHD in
%kids' on the left and `Natural remedies for adhd' on the right.
As can be seen, the first viewport of the SERP is almost completely dominated by sponsored content. 
The vast majority of the sponsored content is highly relevant to ADHD and 
%Not all the sponsored content promotes natural based remedies. 
%One of the ads promotes a non-stimulant prescription medication, two promote treatment programs at private clinics.
%If the parent will try to research natural remedies, they will also be presented
%But most of the ads do 
promotes natural non-prescription products, whose names strongly suggest benefits to attention and focus.
Unfortunately, the fact is that most of these products have not been scientifically proven to be effective \cite{gillies2012polyunsaturated,heirs2007homeopathy}, but this information is not presented next to the ad. Although this information might be included in one of the returned results lower on the page, the parent might not notice them as extra effort is needed to examine those positions \cite{yue2010beyond,joachims2017accurately}. This bias can prevent the parent from making an informed decision that considers all relevant information, which in turn can harm their child ~\cite{harpin2016long}.\footnote{The effective course of treatment for ADHD is out of the scope of this paper.}
%and due to position bias, the probability that the parent will be exposed to it is lower. 

In this work, we explore the effect of sponsored content in search engines on users' decision-making in health related topics, in particular, under the task setting of determining the effectiveness of online available natural remedies to related medical conditions. 
We focus our study on the following research questions: 
\begin{itemize}
    \item \textbf{RQ1:}  How is users’ result examination behaviour affected by the sponsored content on a SERP?
    \item \textbf{RQ2:} When users interact with a search engine to decide about the effectiveness of a medical treatment, does the existence of sponsored content affect their decisions?
   
\end{itemize}

In order to answer these research questions, we conducted a series of user studies in which participants were presented with SERPs discussing the effectiveness of natural remedies on corresponding medical conditions. Participants were presented with a SERP that only included results that specifically discuss the related query but with different viewpoints (e.g., for vs. against).
%meaning that all results were relevant to their query.
The participants were then requested to only use the results presented to them to decide the effectiveness of the remedy mentioned in the query. Each SERP contained an equal number of retrieved results, but the order in which the results with different viewpoints were presented varied so that participants were exposed to different levels of rank bias. 
In the meanwhile, the participants could be presented with a SERP that did not contain any ads, or with an ad that directly markets the remedy discussed in the query, or with an indirect marketing  ad. In particular, indirect marketing is a marketing method in which instead of directly promoting a product or offering it for purchase, the advertisers create promotional content discussing the benefit of the product for the purpose of building the brand. 
%In online advertising, advertisers can mark the user that consumed the promotional content by using cookies and approach them at a later time  using direct marketing. 
%Advertorial ads do not directly recommend that the participant purchase the remedy; instead, their content explicitly supports the effectiveness of the discussed remedy, while direct commerce ads can be embedded within the content of the page. 

We tracked the participants' click behaviour and their responses to our post-study survey questions and compared the results under various settings. % We found that participants perceived direct marketing ads as irrelevant to their information need and mostly disregarded them. 
We found that participants tended to skip direct marketing ads and proceed to organic content. However, the existence of the ads could still affect users' decision making and introduce positive bias. 
For indirect marketing ads, we found that the effect of ads on both participants' examination behaviour and their responses depended on the ranking bias of the organic results. When the organic results were biased towards a negative viewpoint, participants not only skipped the indirect marketing ads during their search but also enforced their negative bias towards the treatment's effectiveness. 
When the organic results were biased towards an inconclusive or positive viewpoint, however, participants were more inclined to inspect the content of the ads which introduced positive bias to their decision making. 
%take the viewpoint presented in it under consideration. 

%The rest of this paper is organized as follow sections XX describes the str

%\begin{figure*}[h]
%\centering
%\begin{subfigure}{0.33\linewidth}
%  \centering
%\includegraphics[scale=0.33,keepaspectratio]{images/omega no ads.pdf}
%  \caption{No Ads}
%  \label{figure:noads}
%\end{subfigure}
%\begin{subfigure}{0.5\linewidth}
%  \centering
%\includegraphics[scale=0.4,keepaspectratio]{images/omega ad.pdf}
%  \caption{Direct Marketing Ads}
%  \label{fig:ads}
%\end{subfigure}%
%\begin{subfigure}{0.5\linewidth}
%  \centering
%\includegraphics[scale=0.4,keepaspectratio]{images/omega sponsored.pdf}
%  \caption{Indirect Marketing Ads}
%  \label{fig:spnsored}
%\end{subfigure}
%\vspace{-3mm}
%\caption{Two possible ad configurations of a SERP for the query:``Do omega fatty acids treat ADHD''}
%\label{fig:ads_conf}
%\vspace{-3mm}
%\end{figure*}

==> Ads paper arXiv/relwork.tex <==

\section{Background and Hypothesis}
We explore the connection between search engine manipulation effect and sponsored content in the health search domain. In this section, we first discuss existing work related to all these aspects
%We will first introduce studies discussing search engine manipulation effect (SEME) in general, followed by discussions about research on search engines' bias in the health domain, and conclude with work focused on the effect of online advertising on users search experience and behaviour. We will 
and then present the null hypotheses related to our research questions.


\noindent\textbf{Impact on Users' Beliefs.} Most studies that explored search engines' effect on users' beliefs and decision-making show that higher ranked results are more likely to affect the users, especially  when the results are biased towards a positive viewpoint~\cite{allam2014impact,pogacar2017positive,epstein2015search,white2014belief}.
One exception to this is ~\cite{draws2021not} who examined the effect of position bias on debatable topics. This study examined the attitude change exhibited in users who held a neutral viewpoint before the study. Although users were affected by the content they read, the data collected by the study showed that despite \textit{position bias}, the order in which results were ranked did not have a significant effect on users' attitude change.

White and Hassan \cite{white2014content} showed that the search results in medical  related queries are often biased toward positive outcomes. White \cite{white2013beliefs} investigated the issue of bias in yes-no question based on online search results about medical conditions. Similar results are observed, showing that users favored more  positive results (irrespective of the truth). More so, White showed that almost half of the times the viewpoints presented in the search results were scientifically incorrect.
Pogacar et al. \cite{pogacar2017positive} presented users with biased SERP and showed that this bias affected users' decision-making in health related questions, and Hashavit et al. ~\cite{hashavit2021understanding} showed that this phenomena repeats even when the users are free to conduct the search on their own.


\noindent\textbf{Impact on Users' Search Experience.} Advertisements' effect on users' search experience has been researched in several studies. Lewandowski at el.
~\cite{lewandowski2017users, lewandowski2018empirical} conducted two large-scale studies on  German internet users that focused on {Google}. Their studies found that users had limited knowledge regarding a search engine's business model. Many of them reported that they were either unaware that it was possible to pay {Google} to present content on the SERP or they did not know how to distinguish between ads and organic results. 
%These results were validated by a task-based user study in which users were asked to mark sponsored content. The authors reported that only a small portion of users were able to distinguish between ads and organic results, and 
Schulthei{\ss} and Lewandowski~\cite{schultheiss2021users} showed that users with less understanding of search engine business models were more likely to click on ads.
%Several eye tracking studies inspected users' attention and reactions to sponsored content when they perform web search ~\cite{giraldo2021influence,alanazi2020impact,buscher2010good,phillips2013ads,lagun2016understanding}.
%~\cite{lagun2016understanding} Found that for shopping intent search, when the ad is relevant to the information need and the ad is of high quality it receives higher attention and improves the search experience.
Several studies found that the quality of ads and their rank affected the attention that ads received as well as the probability the user would click on them~\cite{giraldo2021influence,alanazi2020impact,buscher2010good,phillips2013ads, foulds2021investigating,danescu2010competing,lagun2016understanding}. This correlates with many studies showing users exhibit strong \textit{position bias} towards higher ranked results ~\cite{joachims2017accurately,keane2008people,o2006modeling,pan2007google}. %, meaning that higher ranked results are more likely to be examined and entered by the users.  
However, when examining attention to ads compared to organic results, studies found negative bias toward the sponsored content. Sponsored content received significantly less attention from users in comparison to organic results, and on several occasions they distracted and frustrated the users ~\cite{giraldo2021influence,buscher2010good,foulds2021investigating, danescu2010competing}.
A recent study by Foulds et. al ~\cite{foulds2021investigating} 
%examined multiple aspects of ads effect on users' search performance, experience and behaviour. In this study, participants were asked to collect relevant documents related to a topic they were assigned to. Participants interacted with a news-based retrieval system that returned documents with or without ads depending on the experiment condition. The study 
found that overall ads had a negative impact on users' search experience, their performance in the search task, and their search experience. 

Much research attention has be paid on sponsored content's effectiveness under various conditions from a marketing perspective. The goal of these studies is mainly to examine factors that make advertisement more effective. The main metric inspected is click through rate \cite{jansen2006examination, gauzente2010intention}, some inspect users' attitude towards online advertising \cite{lu2017sponsored} and percentage of successful purchases originated from ads \cite{agarwal2015organic}. These studies focus mainly on e-commerce  and do not explore the effect of sponsored content on users' beliefs.  

To briefly summarize, existing studies examined the effect of ads on users' behaviour and search experience from multiple angles but they did not touch the effect of sponsored content on users' perception or their beliefs. 
%An innate part of marketing campaigns is cognitive change. Before an advertisers can sell their product they must convince users that the need the product. This process  
Our research focuses on not only the effect that ads have on users' search behavior, but also the effect that ads might have on users' decision-making, their beliefs and biases, and their perception of truth in relation to their information need. Previous work in information retrieval suggests users are prone to ignore the ads; but if the users did not pay attention to the search ads, how could the ads be effective in advancing consumer metrics as suggested by studies in marketing science? 
%The possible hypotheses are that user will either: 1)Enter the ads and thus be affected by their content. 2)Enter the ads but remain unaffected by them in their decision making. 3) Skip the ads and thus remain unaffected by their content. And 4) Skip the ads but still be affected by them in their decision making.

%One hypothesis is that, as shown in previous studies, users will not examine the presented ads  and thus not be affected by them in their decision making.Alternatively, they may choose to enter the ads, and get affected in their decision making. Another possibility is, as reported in previous work, %showed users may be affected by ads even if they do not click on them, even though users choose to skip the ads they still get affected by their content. And finally, there is also the possibility that users will examine the ads but will not be affected by them in their decision making, although this hypothesis is not supported by any previous work. 
To understand this seeming contradiction, we phrase two null hypotheses in accordance to our previously defined research questions in the context of health-related search: 
\begin{itemize}
    \item \textbf{H1:}  when sponsored content is presented in the SERP, users will generally skip it and examine mostly organic results, preferring higher ranked results.
    \item \textbf{H2:} when users interact with a search engine to decide about the effectiveness of a medical treatment, the existence of sponsored content will not affect their decision. 
\end{itemize}

We will use the method developed in the next section to carefully study these research questions and verify our hypotheses. 
%~\cite{allam2014impact,pogacar2017positive,white2013beliefs,hashavit2021understanding}
%An issue of great concern ~\cite{wang2019systematic} especially in current time when the world is struggling with the Covid pandemic and accurate medical information can literally save lives. 

%Where previous studies have shown that users are susceptible to positive bias 
%the existence of positive bias in this domain. 
%The existence of search engines 


%present somewhat contradicting results to these studies. Their eye tracking based research conducted on a set of 15 participants showed that users exhibit negative bias towards ads and a preference for organic results Ads can be valuable tools that help users achieve their information need, ~\cite{alanazi2020impact} focus on eye tracking in mobile devices. They found that the users were more likely to select higher rank ads. 



%~\cite{lewandowski2017users} conducted large scale studies on 1000 German internet users that focused on \textit{Google}. The study found that 42\% of users reported that they were either unaware that it is possible to pay \textit{Google} to present content on the SERP or that they did not know how to  These results were later validate by a user study that requested users to mark sponsored content in a SERP. A followup study The same authors concuted another ~\cite{lewandowski2018empirical} conducted large scale studies on 1000 German internet users and found that although users are aware of search engines business model, the vast majority of them struggle to distinguish between organic results and ad.

==> Ads paper arXiv/setup.tex <==
\section{Method and Experimental Setup}
We designed a series of user studies in which participants were required to evaluate the effectiveness of an intentionally selected natural remedy in treating a particular medical condition, only based on the entries in a SERP presented to them.

To this end, we created a dataset of SERPs with a wide variety of viewpoint biases (e.g., supporting or against the natural remedy's effectiveness), different configurations of the SERP (e.g., ranking positions of organic search results, with/without ads) and queries related to different remedies and health conditions. 
Insight regarding users' examination behaviour was collected by tracking users' clicks in their web browsers using JavaScript during the study. Insights regarding users' decision making and their search experience was collected explicitly via a series of survey questions by the end of the study.

%Insight regarding users` exposure behaviour was collected implicitly by tracking users` actions during the survey. Insights regarding decision making and the search experience of users was collected explicitly by requesting participants to answer a series of questions.

%Section \ref{sec: data} describes the data set creating process and section \ref{sec:survey} describes the user study survey. 


\subsection{Dataset Preparation} \label{sec: data}
\subsubsection{Queries}
To conduct our study, we need a set of SERPs related to various queries about natural remedies' effectiveness for a  certain health condition. We chose the following three queries: \label{q:ginkgo} \textbf{Q1:} Ginkgo-biloba for treating tinnitus; \label{q:mlt} \textbf{Q2:} Melatonin for treating jetlag; \label{q:omega} \textbf{Q3:} Omega fatty acids  for treating ADHD.
%\begin{itemize}
%    \item\label{q:ginkgo} \textbf{Q1:} Ginkgo-biloba for treating tinnitus;
%    \item\label{q:mlt} \textbf{Q2:} Melatonin for treating jetlag;
%     \item\label{q:omega} \textbf{Q3:} Omega fatty acids  for treating ADHD.
%\end{itemize}

Each of these three queries has a different ground-truth answer. According to their corresponding Cochrane reviews\footnote{Cochrane \cite{cipriani2011cochrane} is a charity organization whose mission is \say{\textit{to promote evidence-informed health decision-making by producing high-quality, relevant, accessible systematic reviews and other synthesized research evidence.}}
Cochrane only accepts conflict-free funding, so their reviewers can be considered as unbiased.}: Ginkgo biloba is \emph{not effective} in treating tinnitus~\cite{hilton2013ginkgo};  Melatonin is \emph{effective} in treating jet-lag~\cite{herxheimer2002melatonin}; and for omega-3 the answer is inconclusive and further study is required in order to reach a conclusion ~\cite{gillies2012polyunsaturated}. The detailed search result entries were manually retrieved by searching the above queries in well-known search engines. The query phrases entered to the search engines followed patterns that were designed to retrieve relevant results that contain a viewpoint regarding the effectiveness of the treatment for the condition discussed in the query. For example, ``\textit{is melatonin effective for jetlag}'', ``\textit{is melatonin ineffective for jetlag}'' etc.


\subsubsection{Advertisements}

%In total there were 12 possible ranking bias configurations for each query. 
A SERP can have one of three possible ad configurations: 
\begin{enumerate}
    \item Ads clean - no sponsored content at all; 
    \item Direct marketing ads;
    \item Indirect marketing ads. 
\end{enumerate}
 
 
Direct marketing ads are ads that offer the remedy in question for sale. This type of ads refer the users to an online shopping website where they can purchase the remedy. The shopping websites often do not directly discuss the effectiveness of the remedy, in particular not in the title or the snippet of the ads. For example, a direct marketing ad for omega fatty acids had the following title:``\textit{Omega-3 Fish Oil EPA DHA Triple Strength - 2,720 mg - 180...}'', and the following snippet:``\textit{Quality Vitamins \& Supplements Online At Bronson Vitamins. Quality Products Since 1960. 
Save an Additional 10\% To 20\% With Subscribe \& Save Auto Delivery Subscriptions.}''
We hypothesize that the existence of such products might indirectly suggest to users that the product is effective.
Direct marketing ads were retrieved from actual SERPs returned by the commercial search engines.

Indirect marketing ads are entries of sponsored content that contains textual content widely discussing and supporting the use of the remedy for the condition in question. Indirect marketing ads highlight the treatment's effectiveness already in their titles and snippets. For example, an indirect marketing ad for omega fatty acids had the following title: ``\textit{Omega 3s: The Ultimate (ADHD) Brain Food - ADDitude}'', and the following snippet: ``\textit{Supplementing with omega-3s eases hyperactivity. Analyzing data from 16 studies on ADHD and omega-3s, researchers at Oregon Health \& Science ...}'' Although these web pages do not focus on selling the product directly, all of them have links on their websites referring users to a shopping website. Indirect marketing ads were collected from organic search results that were annotated as having a positive viewpoint and containing direct marketing ads for the treatment in question as part of their web page. 
Notice that we excluded third party ad space such as Google AdSense but only considered static commercial content for the treatment in question
%, embedded in the content of the web page, 
when classifying indirect marketing ads.

Our SERPs with sponsored content only included one ad (either direct or indirect marketing ad) placed at the top of the ranked list. Ads were marked by the bold text \textbf{Ad} to the left of their titles, as most commercial search engines would do. 
%Entries that appeared in the sponsored content section did not appear in the organic results section. 
%An example of the two different ad configurations is provided in Figure \ref{fig:ads_conf}. 
The manufactured SERPs resided on our experiment servers but the links to which the users were referred point to actual web pages found online, which we did not alter. 
Since our study's research questions focus on users' perception but not their general search experience, and given the high relevance of commercial search engines in presenting related ads to users, we opted to present only ads that were relevant to the search query at hand.



\subsubsection{Viewpoint Bias}\label{sec:viepoint}
The viewpoint of each entry was independently evaluated by two readers with necessary medical background  knowledge. Entries on which the readers disagreed were removed from the dataset. 
We categorize possible viewpoints into three classes: \emph{supporting (Y)}, \emph{rejecting (N)} and \emph{inconclusive (M)}, in order to coincide with the options later presented to our study participants. 

%We could not find such an entry for the query concerning melatonin as a treatment for jet-lag. We assume that this is because Melatonin is an easily purchased over the counter medication (at least in the US). Therefore our direct marketing content experiments related to queries \ref{q:ginkgo} and \ref{q:omega} from the above list.  




\begin{table}[t]
\caption{Bias level of the various SERP configurations, prior and posterior.}
\vspace{-3mm}
  \begin{tabular}{|c|c|c|c|c|}
    \hline
    Max Bias & B(Y) &B(M)&B(N) & Configurations\\

 \hline
            \multirow{4}{*}{Y} & & & & $y^am^an^a$\\\cline{5-5}
                                & 0.49-0.65 & 0.13-0.29 &0.13-0.29 &  $y^an^am^a$\\\cline{5-5}
             & (0.44-0.56)& (0.18-0.33)& (0.18-0.33)&$(ymn)^a$\\\cline{5-5}
             & & & &{$(ynm)^a$}\\\cline{5-5}             
 \hline
 \hline
            \multirow{4}{*}{M} & & & & $m^ay^an^a$\\\cline{5-5}
                                & 0.13-0.29 & 0.49-0.65 &0.13-0.29 &  $m^an^ay^a$\\\cline{5-5}
             & (0.18-0.33)& (0.44-0.56)& (0.18-0.33)&$(myn)^a$\\\cline{5-5}
             & & & &{$(mny)^a$}\\\cline{5-5}             
 \hline
\hline
            \multirow{4}{*}{N} & & & & $n^ay^am^a$\\\cline{5-5}
                                & 0.13-0.29 & 0.13-0.29 &0.49-0.65 &  $n^am^ay^a$\\\cline{5-5}
             & (0.18-0.33)& (0.18-0.33)& (0.44-0.56)&$(nym)^a$\\\cline{5-5}
             & & & &{$(nmy)^a$}\\\cline{5-5}             
 \hline
\end{tabular}
\label{tab:configs}
\vspace{-4mm}
\end{table}

%\subsubsection{The discussed queries}

%We divided entries viewpoint into three possible results in order to coincide with the options which are available to the participants later, in the survey.

All SERPs had the same number of entries for each of three possible viewpoints to avoid introducing other possible biases. However, they differed in the level of ranking bias induced by their actual rank positions.
We intentionally created two forms of ranking bias: block-wise ranking bias and interleaved ranking bias. In block-wise ranking bias, the viewpoints were divided into three blocks of consecutive result rankings about the same viewpoints. For example, the configuration $yyymmmnnn$ specifies a SERP with 9 results, where three supporting entries are placed in rank position 1-3, three inconclusive results in rank position 4-6, and three rejecting entries in rank position 7-9. 
In interleaved ranking bias, the viewpoints were interleaved with each other. For example, in the configuration $ymnymnymn$, three supporting entries are placed in rank positions \{1,4,7\}, three inconclusive results in rank positions \{2,5,8\} and three rejecting entries in rank positions \{3,6,9\}. We denote a sequence of $a$ consecutive viewpoints of value $v$ as $v^a$, and a sequence of interleaved viewpoints $v_iv_jv_k$ of length $a$ as $(v_iv_jv_k)^a$.
For example, the sequence $yyymmmnnn$ will be denoted as $y^3m^3n^3$ and the sequence $ymnymnymn$ will be denoted as $(ymn)^3$. 

The total a-priori ranking bias of a viewpoint in a SERP can  be viewed as the expected attention that the viewpoint receives.
%, if we assume that the attention that a single document receives is directly proportional to its rank. 
Formally, the ranking bias that viewpoint $v$ expects to receive in a given result ranking $D$ of length $R$ is defined as:
%\begin{equation} \label{eq:bias}
% B(D, v) = \frac{1}{Z}\sum_{i=1}^{R}\frac{1}{i} \mathbbm{1}_{D[i]=v}  
%\end{equation}
\begin{equation} \label{eq:bias}
 B(D, v) = \frac{1}{Z}\sum_{i=1}^{R}P_c(i) \mathbbm{1}_{D[i]=v},
\end{equation}
where $Z$ is a normalization constant,  $\mathbbm{1}_{D[i]=v}$ suggests if the document placed at rank $i$ corresponds to viewpoint $v$ and $P_c(i)$ is the probability of the document to be examined by a user. Given no prior knowledge, we follow the position-based examination model \cite{craswell2008experimental} to estimate the probability by $P_c(i) \propto \frac{1}{i}$.

Table \ref{tab:configs} describes the possible SERP configurations grouped according to the viewpoint which receives the maximal ranking bias.
The first four, the middle four, and the last four are sequences where the maximal bias belongs to the supporting, inconclusive, and rejecting viewpoints respectively. 
The values in columns B(Y), B(M) and B(N) show the ranges of prior and posterior (in parenthesis) bias levels for the configuration associated with each maximal bias viewpoint, as was computed according to Eq \eqref{eq:bias}. 
The posterior bias values will be discussed in the experiment results section: they were calculated based on the actual click-through rate observed in our user study.


In our study the value $a$ was set to either 2 or 3 depending on the number of retrieved result entries for each viewpoint. For query Q1 (`Ginkgo-biloba for treating tinnitus'), we could not find three entries that expressed an inconclusive viewpoint, since its ground-truth is not effective; therefore in order to balance viewpoints, all SERPs for Q1 were limited to 6 results, i.e., $a=2$. For the other queries, $a$ was set to 3. 
For Q2 (`Melatonin for treating jetlag'), we could not find an indirect marketing ad entry. We assume this is because Melatonin can be easily purchased over the counter (at least in the US). Therefore our indirect marketing content experiments were only conducted for query Q1 and Q3.  

For each query there were 12 different bias configurations. For each query-configuration pair, three SERPs were randomly generated. To create the SERP instances with ads, a relevant ad of each type was added to each ad free SERP. In total, 288 SERPs were generated. These basic statistics about our study dataset are summarized in Table \ref{tab:doc_num}. 

 


%Table \ref{tab:configs} describes all possible configurations along with their prior and posterior (in parenthesis) bias values  associated with each possible viewpoint. The posterior bias values will be discussed in the experimental results section, which were calculate based on the actual click-through rate observed in our user study. The first eight rows are sequences where the maximal bias belongs to the supporting viewpoints. The middle eight rows are sequences where the maximal bias belongs to the inconclusive viewpoints, and the last rows are sequences where the maximal bias belongs to the rejecting viewpoints. 


\begin{table}[t]
\caption{Statistics of the user study dataset.}
\vspace{-3mm}
  \begin{tabular}{|l|c|c|c|}
  \hline
  & $Q_1$ & $Q_2$ &$Q3$\\
  \hline
     a&2&3&3\\
    \hline
    \# of entries in a SERP without an ad & 6 &9&9\\
    \hline
    \# of entries in a SERP witho an ad & 7 &10&10\\
    \hline
    \# of SERP bias configurations & 12 & 12& 12\\
    \hline
    \# of SERP instance per configurations & 3& 3& 3\\
    \hline
    Total \# of unique SERPs  & 108& 72& 108\\
  \hline
\end{tabular}
\label{tab:doc_num}
\vspace{-2mm}
\end{table}

\subsection{Variables}
%To summarize, 
The dependant variable in this study is the participants' perceived effectiveness of a natural remedy for a given health condition. It is a categorical variable with three levels: effective, ineffective and inconclusive.  
The independent variables manipulated in our experiments were as follows:
\begin{enumerate}
    \item The discussed query (categorical; between-subjects). Each SERP is about a single query discussing the effectiveness of one treatment for a specific condition. 
    %\item The viewpoint bias presented in the SERP(categorical; between-subjects). A SERP could be bias toward a viewpoint supporting the treatments effectiveness, rejecting its effectiveness (i.e claiming the treatment is ineffective) or an inconclusive viewpoint; for example stating not enough data exists to truly determine if the treatments is effective.
    \item The sponsored content presented in the SERP (categorical; between-subjects).  A SERP could contain a direct marking ad, indirect marketing ad, or no ads at all.
    \item The viewpoint configuration presented in the SERP (categorical; between-subjects). %The viewpoint configuration is the order in which documents viewpoints are presented in the SERP.
    A SERP can take one of 12 possible viewpoint configurations listed in Table \ref{tab:configs}. %Each viewpoint configuration introduces maximum bias towards one of three viewpoints: supporting the treatments effectiveness, rejecting its effectiveness (i.e claiming the treatment is ineffective) or an inconclusive viewpoint; for example stating not enough data exists to truly determine if the treatments is effective. 

\end{enumerate}


\subsection{User Study Procedure} \label{sec:survey}
In this section, we describe the procedure of the user study we conducted.  We used the Amazon Mechanical Turk (MTurk) platform to recruit participants for our study. 
All participants were from English speaking countries. We used MTurk's  external question format which directs participants to the website hosted by our survey web server.
Prior to the beginning of our study, we obtained an institutional review boards (IRB) approval from our institute. 

Upon entering the survey, a participant was requested to provide his/her demographic information, including age, gender, level and field of education. 
After filling in their personal information, the participant was directed to the instruction page. 
At this point, our server assigned a particular SERP instance to the participant. The SERPs were assigned to participants in a round robin manner to ensure a balanced number of responses for each experimental factor. 
%At this point, participants were introduced to the query assigned to them (randomly) and  their task was explained. 
%Since the SERP was already allocated to the participant the instruction referred to the particular query in the assigned SERP. 
Below is an example instruction page discussing the query `Ginkgo biloba for treating tinnitus':
\begin{quote}
Thanks for agreeing to participate in our research survey!
In the next page, you will be presented with a search result page for the query: \textit{is \textbf{Ginkgo biloba} an effective treatment for \textbf{tinnitus}}.
Your task is to determine the answer to this query, \underline{in the context} \underline{of the presented results only.}
Use the search results in the next page (click at least one of results) to find your answer. When you are ready, click the ``Answer Survey'' button to proceed.
\end{quote}


After reading the instructions, participants were asked if they had any previous knowledge regarding the topic of the study. The available options were: 1) yes I do, 2) not a lot, and 3) none. 
We did not want to collect responses that were resulted from the participants' prior knowledge or bias, but we also did not want them to lie in order to participate for payment. Therefore, we did not use this question to filter any participants; and for those who declared having prior knowledge regarding the query, their responses were excluded from the entire analysis of our study (they were still paid for their participation). This was done as part of our study design. %We did not inspect the results of the participants who reported having prior knowledge at any stage.

After answering this question, the participants were referred to the assigned SERP to start the task. 
They were instructed to browse as many links as they needed to answer the question; and they could not progress to the next stage unless they had clicked at least one link. This was to ensure the participants understood that they had to interact with the SERP. 

%When participants felt they were confident enough to answer the survey, they needed to 
Once the participants pressed the ``Answer Survey'' button that was located next to the search box, they were then directed to the question form, where they were required to enter their conclusion regarding the effectiveness of the treatment discussed in the query. The possible answers were: % yes, no, maybe and not-sure. 
\begin{itemize}
    \item No - according to the information I read, it is not effective.
    \item Yes - according to the information I read, it is effective.
    \item Maybe - according to the information I read, it is inconclusive whether or not it is effective.
    \item Not sure - there was not enough information for me to reach a conclusion.
\end{itemize}

In this form, we also included 3 attention questions to filter out careless workers. Participants were required to  1) answer  a multiple choice question about the nature of the remedy that the query was intended for, 2) answer a multiple choice question about the nature of the medical condition that the query concerned, and 3) provide a reason or piece of evidence for their conclusion regarding the remedies' effectiveness. 

%The first two attention questions were multiple choice questions and the third (reason) was an open text question. 
The attention question about the nature of the remedy  was phrased simply as `What is REMEDY'. The available answers for it were:
%The available options for the multiple choice question about the nature of the remedy were: 
\begin{itemize}
    \item A hormone (True for melatonin)
    \item A nutrient found mostly in fish, nuts and seeds (True for omega fatty acids)
    \item A tree (True for Ginkgo biloba)
\end{itemize}

The attention question about the nature of the medical condition was phrased simply as `What is MEDICAL CONDITION'. The available answers for it were:
%The available options for the multiple choice question about the nature of the medical condition  were: 
\begin{itemize}
    \item A neurological disorder (True for ADHD)
    \item Ringing noise in one or both ears (True for tinnitus)
    \item A sleep problem (True for jet-lag)
\end{itemize}

Participants who did not answer the filter questions correctly or did not provide a coherent reason for their choice, were removed from the analysis.
Participants were also provided with the opportunity to add general comments about the study itself. By the end of our study, we received very positive feedback from the participants, indicating that the survey instructions were clear and the task  was easy to follow. Several participants noted that they liked the survey and it was interesting to them. 

Once participants submitted their answer about the treatments' effectiveness and attention questions, they could not go back and alter them. 
If the SERP presented to the participants included ads, they were presented with two additional questions about the influence of the ad to their overall search experience and to their decision about the treatment's effectiveness. Participants were also allowed to enter any general comments concerning the ad. 
%The responses to both questions were measured by a 5-point Likert scale which ranged from -2 to +2. 
The first question %was about the ad's effect on the participant's search experience. It 
was phrased as:
``The search result page you viewed contained sponsored content (Ads). How much did the ad affect your search experience?''
The responses to this question were measured by a 5-point Likert scale which ranged from -2 to +2, with negative values indicating the ads worsened the search experience and positive values indicating it improved it.
%The possible answers were as follows:
%\begin{itemize}
%    \item -2: It worsened my experience significantly.
%    \item -1: It worsened my experience a little.
%    \item 0: It made no difference.
%    \item +1: It improved my experience a little.
%    \item +2: It improved my experience significantly.
%\end{itemize}
The second question was 
%about the ad's effect on participant's decision regarding the treatment's effectiveness. It was
phrased as: ``How much did the ad affect your decision regarding the treatment's effectiveness?'' We again used a 5-point Likert scale with negative values indicating the ads added doubts to participants' decisions and positive values indicating ads enhanced their belief in their decision. % The possible answers were:
%\begin{itemize}
%    \item -2: It added serious doubts.
%    \item -1: It added some doubts.
%    \item 0: It made no difference.
%    \item +1: It slightly enhanced my %belief. 
%    \item +2: It significantly enhanced my belief.
%\end{itemize}

Once the participants answered all of the survey's questions, they would receive a verification code to receive their payment from the MTurk website. Since our study is between subject, each participant was exposed to only one SERP. Once a participant completed the task, they were not offered to take the survey again. 
On this page, they were also presented with a highlighted warning message noting that they were participating in an experiment and should not make any real conclusions as to the true effectiveness of the remedy discussed in the query.

Participants were paid at a basis rate of \$1 for participation. In addition, they were informed that they would receive a \$1 bonus if their answers were qualified based on their logged search behaviors. By our design, to receive the bonus they had to answer our post survey attention questions correctly and spend at least two minutes on the task itself. 
The payment scheme was derived from a preliminary experiment run in our lab by volunteers that were not MTurk workers, in order to estimate the time it takes to complete the survey task. We added additional time to account for slower working participants, in order to make sure we comply with an hourly payment of at least the US minimum wage. A later analysis of the average time it took the actual participants to complete the task reveled that this was indeed the case.



%For each of the 16 configurations with a maximal bias towards an inconclusive or negative viewpoint a corresponding configuration 
%since these sequences already possessed a strong bias towards a positive result and all types of ads can be considered as expressing a supportive viewpoint 

==> archive.tex <==


%\begin{table}
%\caption{T-Tests comparisons between the different answers for all ad-bias configurations}
%\vspace{-1mm}
% \begin{tabular}{|c|c|c|c|c|}
%\cline{2-5}
%\multicolumn{1}{c|}{}&\thead{df}&\thead{Yes-\\Maybe}&\thead{Yes-\\No}&\thead{Maybe-\\No}\\
%\hline
%\textbf{Y}&53&t=4.31,p < 0.01&t=4.72,p < 0.01&t=1.43,p > 0.05\\
%\hline
%\textbf{AY}&32&t=1.00,p > 0.05&t=4.00,p < 0.01&t=3.73,p < 0.01\\
%\hline
%\textbf{SY}&33&t=-1.00,p > 0.05&t=3.45,p < 0.01&t=3.71,p < 0.01\\
%\hline
%\hline
%\textbf{M}&49&t=-4.15,p < 0.01&t=-1.00,p > 0.05&t=3.93,p < 0.01\\
%\hline
%\textbf{AM}&42&t=-3.33,p < 0.01&t=-1.00,p > 0.05&t=3.10,p < 0.01\\
%\hline
%\textbf{SM}&63&t=-1.43,p > 0.05&t=4.01,p < 0.01&t=4.39,p < 0.01\\
%\hline
%\hline
%\textbf{N}&49&t=-4.58,p < 0.01&t=-4.37,p < 0.01&t=1.00,p > 0.05\\
%\hline
%\textbf{AN}&45&t=-2.60,p < 0.05&t=-3.54,p < 0.01&t=-2.07,p < 0.05\\
%\hline
%\textbf{SN}&51&t=-2.33,p < 0.05&t=-5.65,p < 0.01&t=-4.55,p < 0.01\\
%\hline
%\end{tabular}
%\label{tab:ttest}
%\vspace{-3mm}
%\end{table}



%When the maximal bias level of SERPs is towards the negative viewpoint we see that when no ads are present the `No' and and `Maybe' answers receive a similar percentage of the answers while the `Yes' answer receives a significantly lower percentage. Indicating that partipants had a difficult time interpreting the negative content. When referring to scientific evidence, as in query topics discussed in this study, negative content can often discuss existing positive findings while presenting an overall negative conclusion. This can confuse layman readers. For direct marketing ads we see a similar portion of negative answers but the division of the remaining responses is no longer similar with the `Maybe' response receiving significantly higher portion of the responses in comparison to the `Yes' answer. We see a similar phenomena in the indirect marketing ads setting. However, in this setting we see an significant increase in the portion of users selecting ``No'', both in comparison to the other two answers and to the portion of users selecting ``No'' in the no ads and direct marketing ads configuration. We hypothesis that the difference between the reaction to both ad types stems from the explicit nature of indirect marketing which had a different effect of partipants that were perhaps dangling between two possible answers. Since direct marketing ads don't explicitly express an opinion regarding treatments' effectiveness they did not elicit significant negative bias with those unsure partipants.Participants that were otherwise inclined to select ``Maybe'', perhaps dangling between ``Yes'' and ``Maybe'', were positively affected by the ad and chose ``Yes''. As opposed to indirect marketing ads that explicitly praised the treatment, in the title and snippet of their sponsored web page, causing those dangling  between ``Maybe'' and ``No'' to choose no.  

 

%existence of the indirect marketing content introduced negative sentiments to partipants, causing those unsure partipants, that might have chosen a ``Maybe'' response in the No ads configuration, to opt for the ``No'' response.  
%Though according to the CTR information for negative bias SERPs both the direct or indirect marketing ads were generally skipped.

%Unlike the the positive and inconclusive bias, where the no ads configuration the most popular response correlated to the viewpoint bias. 




%When the maximal bias level is towards the positive viewpoint and no ads are present the ``Yes'' answer is chosen by most participants at a percentage which is quite higher than that of partipants that chose either ``Maybe'' or ``No''. . A different behaviour is exhibited when ads are present. In both the direct and indirect marketing ad configurations, we see a  higher portion of partipants choosing the ``Maybe'' in comparison to the no ads configurations. This difference is  weakly significant in the direct marketing ads configuration t(85.0)=-1.6, p=0.056,  and strongly significant difference in the indirect marketing ads configuration t(86.0)=-1.78, p=0.039.  These results indicate that for positive bias SERPs, where the viewpoint presented by the ads correlates to viewpoint ranking bias expressed in the SERP, participants that consumed negative viewpoint content were effected not only by the ranking bias of the SERP in general but also by the ads and opted for a ``Maybe'' response more frequently.  And this occurred  whether or not they consumed the content in the ad. 



%When the maximal bias level of SERPs is towards the inconclusive viewpoint we see that when no ads are present the correlating `Maybe' response received the highest portion of answers.  When examining the ads configurations for this bias level, we see different behaviours between the direct and indirect marketing configuration. When direct marketing ads are present we see a similar behaviour to that of the no ads configuration. However for the indirect marketing ads we see that the ``Yes'' response receives a significantly higher portion of responses in comparison toe the no ads configuration, t(112.0)=-1.71, p=0.045.We hypothesize that since the viewpoint of the SERP was not definite, participants were not effected by direct marketing ads. This might be due to to the fact that its opinion regarding the treatments effectiveness is very implicit. They were however effected by the indirect marketing ads where we see a lower percentage of negative answers and a higher percentage of positive answers.
%We see a general shift towards more positive answers. We hypothesise that participants that were exposed to the ad in addition to negative content were more likely to chose the `'Maybe'' answer and participants that exposed to the ad in addition to inconclusive results were more prone to choose ``Yes''.

%When the maximal bias level of SERPs is towards the negative viewpoint we see that when no ads are present the `No' and and `Maybe' answers receive a similar percentage of the answers while the `Yes' answer receives a significantly lower percentage.  For direct marketing ads we do not see any sadistically significant difference between the different response percentages. However, for indirect marketing ads we see a weakly significantly higher percentage of negative responses in comparison to that of the no ads configuration. t(100)=-1.4,p=0.08 and a strongly significant for the `Maybe' response t(100)=1.8,p=0.04. This, despite of the fact that according to the CTR information for negative bias SERPs both the direct or indirect marketing ads were generally skipped. Meaning that the indirect marketing ad invoked a negative sentiment amongst partipants that caused partipants that were exposed to inconclusive content opted to select a negative answer more often, simply by noticing that the ad existed, event without inspecting it. This did not occur in the direct marketing setting. In fact we even see a slighr inclination towards a more positive restuls 


%Despite the fact that according to the CTR data, participants did enter the sponsored and the sponsored content expressed the same viewpoint as the organic result. The meet fact that sponsored content existed in the SERP. When an ad is present the rank of each organic results is pushed one position down. Before encounterin a negative or an oncoclusive result viewpoint the partipant is present with ate least one positove viewpoint results and the ad which is also considred as intoducing a positive viewpoint. Since there is no contradiction between the viewpoint bias presented in teh SERP, even when the ad is direct, and despite the fact that according to our CTR inforamtion it is genrally skipped, it effects the decisions of users that are more prone to chose `Maybe' in comparison to `No' in comparison to the equivalent no ad configuartion. When an indirect marketing ad is present we see a similar behaviour. The suprising result here as that the ads had a similar effect eventhtough their CTR data is different. The direct ads were genralky skipped while the indirect ads were often inspected. Showing that the effect ads have on users is not lmited to users that chose to enter the ad. Merly noticing that its their already introduces a shift in the users` thought process. 


%We continue to inspect SERPs   with a bias towards the inconclusive viewpoint we again see, as expected, that the highest portion of partipants chose the correlating `Maybe' answer for all add configurations. Here too we see a slight decline of the portion of partipants that chose this answer when ads are present. For direct marketing ads, this decrease in divided equally between the two other answer that exhibit a slight increase of 2\% each in comparison to their correlating answer in the no ad configuration. For indirect marketing ads we see a different behaviour with the `Maybe' answer receiving We again see a similar percentage of responses for the `Maybe' and `Yes' responses, this unlike the no marketing and direct marketing ads configuration in which `No' and `Maybe' answers are the ones that receives a similar percentage of the results. This differences are supported by users' examination behaviour. When the ads were direct they users did not enter them and therefore were not greatly influenced by them, but when the ads were indirect, they did choose to enter them and were influenced by them and therefore chose to answer `Yes' more often. Finally we inspect SERPs with a bias towards a negative viewpoint. Here we see that when no ads are present, unlike in the previous viewpoint bias configuration, the result do not correlate to the maximal bias level, with the `Maybe' option receiving the highest portion of answers. This result is explained by peoples general preference to favour positive results. When ads are not present   we see a similar distribution of the `Maybe' and `No' answers, both of tehm are significantly higher than the 14\% poistive responses.  For direct marketing ads we see a similar portion of negative responses For indirect marketing ads we see a high increse of 14\% in the porecentage of negative responses, more than twice the precentege of the `Maybe' response and three tiems the precentage of positive responses. 

%\renewcommand{\arraystretch}{1.35}
%\begin{table}[t]
%\caption{Statistics about the estimated regression weights.}
%\vspace{-2mm}
%\begin{tabular}{|l|c|c|c|c|c| } 
%\hline
%\textbf{Type} & \textbf{Response} &\textbf{\# Non-Zero} &\textbf{Min}&\textbf{Max}\\
%\hline 
%No Ads&Y&9&-1.69 ($^3_M$)&1.15 ($^1_Y$)\\
%\hline 
%No Ads&M&10&0.03 ($^6_N$)&0.89 ($^1_M$)\\
%\hline 
%No Ads&N&13&-1.88 ($^2_Y$)&2.45 ($^8_N$)\\
%\hline
%DM&Y&9&-2.02 ($^3_N$)&1.65 ($^5_Y$)\\
%\hline
%DM&M&7&-0.46 ($^3_N$)&0.81 ($^3_M$)\\
%\hline
%DM&N&11&-1.36 ($^4_Y$)&1.44 ($^5_N$)\\
%\hline
%IM&Y&8&-2.24 ($^4_M$)&1.64 ($^1_S$)\\
%\hline
%IM&M&4&0.10 ($^2_N$)&1.45 ($^6_N$)\\
%\hline
%IM&N&9&-0.41 ($^4_M$) &1.72 ($^2_N$)\\
% \hline
%\end{tabular}
%\label{tab:weight_stats}
%\vspace{-3mm}
%\end{table}

